Beyond Generalization: A Survey of Out-Of-Distribution Adaptation on Graphs

Distribution shifts on graphs -- the data distribution discrepancies between training and testing a graph machine learning model, are often ubiquitous and unavoidable in real-world scenarios. Such shifts may severely deteriorate the performance of the model, posing significant challenges for reliable graph machine learning. Consequently, there has been a surge in research on graph Out-Of-Distribution (OOD) adaptation methods that aim to mitigate the distribution shifts and adapt the knowledge from one distribution to another. In our survey, we provide an up-to-date and forward-looking review of graph OOD adaptation methods, covering two main problem scenarios including training-time as well as test-time graph OOD adaptation. We start by formally formulating the two problems and then discuss different types of distribution shifts on graphs. Based on our proposed taxonomy for graph OOD adaptation, we systematically categorize the existing methods according to their learning paradigm and investigate the techniques behind them. Finally, we point out promising research directions and the corresponding challenges. We also provide a continuously updated reading list at https://github.com/kaize0409/Awesome-Graph-OOD-Adaptation.git

==> 5OOD.tex <==
\section{Graph OOD Generalization}
\label{sec:OOD}
In the context of graph OOD generalization, the setting is notably more challenging as target samples are not pre-collected in advance.
The best one can do is to enhance the overall generalizability of the model, such that it can handle samples from any unseen domain.
In this section, we briefly discuss graph OOD generalization, providing a big picture of the field and highlighting the most recent updates.
For a more comprehensive review, we refer readers to the survey on graph OOD generalization \cite{Li2022OutOfDistributionGO}.

\subsection{Model-Centric Approach}
\kz{another work: HANDLING DISTRIBUTION SHIFTS ON GRAPHS: AN INVARIANCE PERSPECTIVE}
\sh{There are a lot of works like this in the survey paper \cite{Li2022OutOfDistributionGO}. I only covered the newest papers. Do I need to add more here?} \\
\smallskip 
\noindent
\textbf{Graph invariant learning}, aiming to capture the invariant relationships between inputs and labels across different environments, is undoubtedly the most popular method for graph OOD generalization.
In general, graph invariant learning learns the invariant graph pattern or property across different environments based on causality-based principles, or bi-level worst-case risk minimization, or explicit alignment regularization \cite{Li2022OutOfDistributionGO}. 
Very recently, authors \cite{Gui2023Joint} identify two stages of environment-based methods, namely environmental inference stage and environmental exploitation stage, where the first phase involves inferring the environmental labels and the second phase focuses on utilizing the acquired environmental labels effectively. 
While many attentions have been paid for graph-specific environmental inference, environmental exploitation are relatively less studied for graph structured data.
To make full use of label and environment information, they introduce LECI (label and environment independence), and incorporate the two causal independence principles in subgraph discovery framework. 
As for environmental inference, recent work \cite{Chen2023Does}
provides an in-depth analysis for the ‘no free lunch’ dilemma, namely 
it’s infeasible to learn invariant graph representations via environment augmentation without additional assumption. 
They further establish the minimal assumption for feasible invariant learning and develop graph invariant learning assistant framework.

\smallskip
\noindent
\textbf{Other learning strategies}
are also used for enhancing the generalizability of representation learning in graph OOD generalization, such as multi-task and multi-view learning \cite{Hu2019StrategiesFP}, contrastive learning \cite{You2020GraphCL}, disentangled learning \cite{yang2020factorizable}, and meta-learning \cite{Lin2023Multi}. \kz{adversarial training?}



\subsection{Data-Centric Approach}
\smallskip
\noindent
\textbf{Data augmentation:}\kz{not consistent with previous sections}
\sh{why is it not consistent}
\textbf{Data augmentation:}
It's widely accepted that the generalization ability of a model heavily relies on the diversity and quantity of the training data \cite{Wang2021Gen}. 
One intuitive yet efficient way to boost the model's generalizability is to increase the diversity of training data through graph data augmentation. 
Typically, graph data augmentation can be categorized based on the augmentation modality as structure-wise augmentations, feature-wise augmentations, and mixed-type augmentations \cite{Li2022OutOfDistributionGO}. 
Upon the diverse graph augmentation methods, recent works shed light on maintaining the invariant rationale during augmentation.  
Authors \cite{Yu2023MindTL} notice that graph labels may be changed during graph structural edition, and propose LiSA to avoid the label shift issue during graph augmentation.
A variational subgraph generator is trained to produce label-invariant subgraphs, which are subsequently used in aiding graph OOD generalization.
AIA \cite{Sui2023Unleashing} is proposed to deal with the graph covariate shift through adversarial graph data augmentation. 
Specifically, the stable features are identified from the data and maintained during augmentation.
G-Splice and FeatX \cite{Li2023GraphSA}, environment-aware structure and feature linear extrapolation are also designed to augment graph data without corrupting the underlying causal mechanisms related to the labels.




